CircuitFusion: Multimodal Circuit Representation Learning for Agile Chip Design

The rapid advancements of AI rely on the support of ICs. However, the growing complexity of digital ICs makes the traditional IC design process costly and time-consuming. In recent years, AI-assisted IC design methods have demonstrated great potential, but most methods are task-specific or focus solely on the circuit structure in graph format, overlooking other circuit modalities with rich functional information. In this paper, we introduce CircuitFusion, the first multimodal and implementation-aware circuit encoder. It encodes circuits into general representations that support different downstream circuit design tasks. To learn from circuits, we propose to fuse three circuit modalities: hardware code, structural graph, and functionality summary. More importantly, we identify four unique properties of circuits: parallel execution, functional equivalent transformation, multiple design stages, and circuit reusability. Based on these properties, we propose new strategies for both the development and application of CircuitFusion: 1) During circuit preprocessing, utilizing the parallel nature of circuits, we split each circuit into multiple sub-circuits based on sequential-element boundaries, each sub-circuit in three modalities. 2) During CircuitFusion pre-training, we introduce three self-supervised tasks that utilize equivalent transformations both within and across modalities. 3) When applying CircuitFusion to downstream tasks, we propose a new retrieval-augmented inference method, which retrieves similar known circuits as a reference for predictions. It improves fine-tuning performance and even enables zero-shot inference. Evaluated on five different circuit design tasks, CircuitFusion consistently outperforms the SOTA supervised method specifically developed for every single task, demonstrating its generalizability and ability to learn circuits' inherent properties.

==> section/bak.tex <==
\textbf{Hardware circuit representation learning}
The distinct mechanisms of HDL compared to traditional PLs make existing PL encoders suboptimal for HDL, raising the need for developing hardware-specific representation learning methods.
In recent years, there has been work exploring the learning of representations for circuit designs~\cite{} to assist downstream EDA tasks, such as design quality prediction~\cite{}, circuit functional reasoning~\cite{}, and verification~\cite{}. 
Most methods utilize the structure of the circuit, converting RTL or netlist designs into graph
format, and then capture the semantic information on the graphs utilizing task-related supervisions or self-supervised graph contrastive learning.



Code representation learning converts source code into informative embeddings that capture the essential semantics and structure of the code. This field plays a pivotal role in enabling various applications, such as automated code analysis~\cite{}, semantic code search~\cite{}, and software defect prediction~\cite{}. Recent advancements have focused on developing encoder models specifically tailored to source code corpora, with the capability to generalize across multiple programming languages (PLs). However, most existing general-purpose code representation methods are specifically designed for the software PLs, neglecting hardware description languages (HDLs) for hardware circuits. 



\textbf{Limitations}
However, we argue that focusing exclusively on the graph modality restricts the ability to fully capture the semantics of hardware circuits. Especially for the RTL-stage HDL code, the raw HDL code contains rich semantic and functional behavior information. While some work has explored incorporating token embeddings of HDL code into graph node features~\cite{}, these approaches do not involve deep multimodal fusion for comprehensive HDL code representation learning. Additionally, in a typical design flow, earlier design stages (i.e., higher abstraction levels) capture more semantic content, while later stages (i.e., lower abstraction levels) introduce complex implementation details. Aligning representations across these design stages would significantly enhance the richness of the learned representations. However, existing methods have not yet addressed the challenge of capturing circuit information across different design stages.


\iffalse
\textbf{Learning software code, as a reference.} As for another popular code format, software programming language (PL), there have been more explorations in developing encoders~\citep{feng2020codebert,guo2020graphcodebert,guo2022unixcoder, li2023starcoder, 
wang2023codet5+,
zhang2024code}, %to capture syntactic and semantic code information. %These encoders enable various applications, such as
enabling automated code analysis, semantic code search, software defect prediction, etc. These encoders also consider different modalities of software code, including the code context, graph structure, and descriptions in natural language. \textbf{However, there are significant differences between the core underlying mechanisms of software PLs and hardware HDLs}, as we will introduce below.  
\fi



\subsection{Few-Shot and Zero-Shot Prediction}


\begin{figure}[!h]
  \centering
  \includegraphics[width=1\linewidth]{./fig/fewshot.pdf}
    % \vspace{-.2in}
  \caption{Zero-shot and few-shot inference of CircuitFusion.}
  \label{fig:fewshot}
  \vspace{-.05in}
\end{figure}



\Cref{fig:fewshot} illustrates the performance of CircuitFusion compared to SOTA baselines for zero-shot and few-shot learning on five design quality prediction tasks. The baseline method is selected as the top-performing model from all baselines in~\Cref{tbl:sft}.
The x-axis represents the fraction of training data used, ranging from zero-shot (0) to full-shot (1), while the y-axis shows the MAPE. These results demonstrate CircuitFusion’s effectiveness in both zero-shot and few-shot settings, making it a versatile and reliable model for early-stage design quality prediction tasks, where access to large datasets is often restricted.

\textbf{Zero-shot.}
Only CircuitFusion supports this zero-shot capability due to our innovative retrieval-augmented method. While the baselines do not provide predictions in the zero-shot setting, CircuitFusion achieves reasonable prediction accuracy without any training data, demonstrating its unique advantage.

We also provide a detailed evaluation of how the number of retrievals affects the prediction results, as shown in~\Cref{tbl:retrieve}. CircuitFusion consistently performs best at top-1 retrieval for all tasks, achieving the lowest MAPE across the board. 
This result indicates that the encoded HDL embeddings contain rich semantic circuit information, enabling effective search and differentiation of functionally similar circuits.
In contrast, other general text or software code encoders struggle to identify functionally similar HDL code snippets. This gap highlights the limitations of models that are not tailored to hardware design, emphasizing the importance of integrating hardware-specific properties into HDL code learning.



\textbf{Few-shot.}
CircuitFusion is particularly effective when training data is limited, which is crucial given the data availability challenges in hardware circuit design. As more training data is introduced (from 1/8 to full-shot), CircuitFusion consistently outperforms the baselines across all tasks, showing steeper performance improvements. It achieves lower MAPEs in nearly all cases, highlighting its superior ability to generalize and learn with minimal data.

